I$^3$Net: Inter-Intra-slice Interpolation Network for Medical Slice Synthesis

Medical imaging is limited by acquisition time and scanning equipment. CT and MR volumes, reconstructed with thicker slices, are anisotropic with high in-plane resolution and low through-plane resolution. We reveal an intriguing phenomenon that due to the mentioned nature of data, performing slice-wise interpolation from the axial view can yield greater benefits than performing super-resolution from other views. Based on this observation, we propose an Inter-Intra-slice Interpolation Network (I$^3$Net), which fully explores information from high in-plane resolution and compensates for low through-plane resolution. The through-plane branch supplements the limited information contained in low through-plane resolution from high in-plane resolution and enables continual and diverse feature learning. In-plane branch transforms features to the frequency domain and enforces an equal learning opportunity for all frequency bands in a global context learning paradigm. We further propose a cross-view block to take advantage of the information from all three views online. Extensive experiments on two public datasets demonstrate the effectiveness of I$^3$Net, and noticeably outperforms state-of-the-art super-resolution, video frame interpolation and slice interpolation methods by a large margin. We achieve 43.90dB in PSNR, with at least 1.14dB improvement under the upscale factor of $\times$2 on MSD dataset with faster inference. Code is available at https://github.com/DeepMed-Lab-ECNU/Medical-Image-Reconstruction.

==> tables/eg.tex <==

\begin{table}
\caption{Units for Magnetic Properties}
\label{table}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{|p{25pt}|p{75pt}|p{115pt}|}
\hline
Symbol& 
Quantity& 
Conversion from Gaussian and \par CGS EMU to SI $^{\mathrm{a}}$ \\
\hline
$\Phi $& 
magnetic flux& 
1 Mx $\to  10^{-8}$ Wb $= 10^{-8}$ V$\cdot $s \\
$B$& 
magnetic flux density, \par magnetic induction& 
1 G $\to  10^{-4}$ T $= 10^{-4}$ Wb/m$^{2}$ \\
$H$& 
magnetic field strength& 
1 Oe $\to  10^{3}/(4\pi )$ A/m \\
$m$& 
magnetic moment& 
1 erg/G $=$ 1 emu \par $\to 10^{-3}$ A$\cdot $m$^{2} = 10^{-3}$ J/T \\
$M$& 
magnetization& 
1 erg/(G$\cdot $cm$^{3}) =$ 1 emu/cm$^{3}$ \par $\to 10^{3}$ A/m \\
4$\pi M$& 
magnetization& 
1 G $\to  10^{3}/(4\pi )$ A/m \\
$\sigma $& 
specific magnetization& 
1 erg/(G$\cdot $g) $=$ 1 emu/g $\to $ 1 A$\cdot $m$^{2}$/kg \\
$j$& 
magnetic dipole \par moment& 
1 erg/G $=$ 1 emu \par $\to 4\pi \times  10^{-10}$ Wb$\cdot $m \\
$J$& 
magnetic polarization& 
1 erg/(G$\cdot $cm$^{3}) =$ 1 emu/cm$^{3}$ \par $\to 4\pi \times  10^{-4}$ T \\
$\chi , \kappa $& 
susceptibility& 
1 $\to  4\pi $ \\
$\chi_{\rho }$& 
mass susceptibility& 
1 cm$^{3}$/g $\to  4\pi \times  10^{-3}$ m$^{3}$/kg \\
$\mu $& 
permeability& 
1 $\to  4\pi \times  10^{-7}$ H/m \par $= 4\pi \times  10^{-7}$ Wb/(A$\cdot $m) \\
$\mu_{r}$& 
relative permeability& 
$\mu \to \mu_{r}$ \\
$w, W$& 
energy density& 
1 erg/cm$^{3} \to  10^{-1}$ J/m$^{3}$ \\
$N, D$& 
demagnetizing factor& 
1 $\to  1/(4\pi )$ \\
\hline
\multicolumn{3}{p{251pt}}{Vertical lines are optional in tables. Statements that serve as captions for 
the entire table do not need footnote letters. }\\
\multicolumn{3}{p{251pt}}{$^{\mathrm{a}}$Gaussian units are the same as cg emu for magnetostatics; Mx 
$=$ maxwell, G $=$ gauss, Oe $=$ oersted; Wb $=$ weber, V $=$ volt, s $=$ 
second, T $=$ tesla, m $=$ meter, A $=$ ampere, J $=$ joule, kg $=$ 
kilogram, H $=$ henry.}
\end{tabular}
\label{tab1}
\end{table}

==> tables/tab_abl_all.tex <==
\begin{table}[t]
\renewcommand\arraystretch{1.1}
\centering
    \caption{Effectiveness of different modules in the whole network. All experiments are conducted using colon dataset with $\times$2 upscale factor.}
    \label{tab:abl_all}
    \setlength{\tabcolsep}{1mm}{
    
    \begin{tabular}{|ccc|cc|}
        \hline
        Intra-slice Branch & Inter-slice Branch & \blue{Cross-view Block} & PSNR & SSIM$_\textrm{a}$ \\ \hline
          &  &  & 42.40 & 0.9841 \\ 
        \checkmark &  &  & 42.89 & 0.9851 \\ 
        \checkmark & \checkmark & & 43.72 & 0.9857 \\ 
        \checkmark & \checkmark & \checkmark & \textbf{43.90} & \textbf{0.9871} \\  
        \hline
    \end{tabular}
    }
\end{table}

==> tables/tab_abl_numOfBlocks.tex <==

\begin{table}[b]\color{blue}

\renewcommand\arraystretch{1.1}
\centering
\caption{{\color{blue}Different number of I$^2$Blocks. All experiments are conducted using colon dataset with $\times$2 upscale factor.}}
        \centering
		% \begin{tabular}{|c|ccccc|}
        % \setlength{\tabcolsep}{2mm}{
        \begin{tabular}{|p{20mm}|ccccc|}
                \hline
                \centering I$^2$Block & 8 & 12& 16 & 20 & 24 \\ \hline
                \centering w CVB   &  43.52 & 43.76 & 43.90 & 43.95 & 44.02 \\ 
                \centering w/o CVB &  43.38 & 43.62 & 43.72 & 43.72 & 43.84 \\  \hline
                \centering $\Delta$ & +0.14 & +0.14 & +0.18 & +0.23 & +0.18 \\
                \hline
		\end{tabular}
\label{tab:abl_num_i2block}
\end{table}

\begin{table}[b]\color{blue}
\renewcommand\arraystretch{1.1}
\centering
\caption{{\color{blue}Different number of Cross-view Blocks. All experiments are conducted using colon dataset with $\times$2 upscale factor.}}

\subfloat{
        % \setlength{\tabcolsep}{2mm}{
		\begin{tabular}{|p{20mm}|ccccc|}
                \hline
                \centering CVB  & 0 & 1 & 3 & 5 & 9 \\ \hline
                \centering PSNR & 43.72 & 43.85 & 43.90 & 43.86 & 43.83 \\ 
                \hline
		\end{tabular}
        }
\label{tab:abl_num_cvb}
\end{table}

==> tables/tab_contrastive_learning.tex <==
\begin{table}[t]\color{blue}
\renewcommand\arraystretch{1}
\centering
    \caption{\blue{PSNR results of two contrastive learning stratgies with different wight $w$.}}
    \label{tab:contrastive_learning}
    \setlength{\tabcolsep}{3mm}{
    \begin{tabular}{|p{5mm}|ccccc|}
        \hline
        \centering $w$ & 0     & 0.05   & 0.10   & 0.20 & 0.50 \\ \hline
        \centering $\mathcal{L}_{c,1}$   & 43.90 & 43.88 & 43.92 & 43.88 & 43.75 \\ 
        \centering $\mathcal{L}_{c,2}$   & 43.90 & 41.38 & 41.04 & 40.73 & 40.18 \\ 
        \hline
    \end{tabular}
    }
\end{table}
